PriMeSRL-Eval: A Practical Quality Metric for Semantic Role Labeling Systems Evaluation

Semantic role labeling (SRL) identifies the predicate-argument structure in a sentence. This task is usually accomplished in four steps: predicate identification, predicate sense disambiguation, argument identification, and argument classification. Errors introduced at one step propagate to later steps. Unfortunately, the existing SRL evaluation scripts do not consider the full effect of this error propagation aspect. They either evaluate arguments independent of predicate sense (CoNLL09) or do not evaluate predicate sense at all (CoNLL05), yielding an inaccurate SRL model performance on the argument classification task. In this paper, we address key practical issues with existing evaluation scripts and propose a more strict SRL evaluation metric PriMeSRL. We observe that by employing PriMeSRL, the quality evaluation of all SoTA SRL models drops significantly, and their relative rankings also change. We also show that PriMeSRLsuccessfully penalizes actual failures in SoTA SRL models.

==> Performance measure metric for SRL/compare_table.tex <==

%%% First comparison table
\begin{table*}[tbhp]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccllllllllll}
\toprule
\multirow{3}{*}{Model}        & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Evaluation\\ script\end{tabular}}   & \multicolumn{5}{c}{In-domain}                       & \multicolumn{5}{c}{Out-of-domain}                    \\ \cmidrule(lr){3-7} \cmidrule(lr){8-12}
                              &                              & \multicolumn{1}{c}{PSD}   & \multicolumn{3}{c}{Argument Classification} &    & \multicolumn{1}{c}{PSD}    & \multicolumn{3}{c}{Argument Classification}     & \\  \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){8-8} \cmidrule(lr){9-11}
                              &                              & \multicolumn{1}{c}{F1}    & P             & R            & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{(r)}       & \multicolumn{1}{c}{F1}     & P             & R            & \multicolumn{1}{c}{F1}   & \multicolumn{1}{c}{(r)}        \\ \midrule
                              
\multirow{2}{*}{\cite{conia-etal-2021-unifying}} & \multicolumn{1}{l}{CoNLL09}  & 96.9  & 89.5          & 89.5         & 89.5    & (3)    & 87.8   & 82.0          & 81.9         & 81.9 & (3)        \\
& \shortprop & 95.5($\downarrow$\red{1.4})  & 86.6          & 86.6         & 86.6($\downarrow$\red{2.9}) & (2)        & 80.9($\downarrow$\red{6.9})   & 72.4         & 72.6         & 72.5($\downarrow$\red{9.4})  & (4)  \\  \cmidrule{2-12}

\multirow{2}{*}{\cite{blloshmi2021generating}$_{\text{nested}}$} & \multicolumn{1}{l}{CoNLL09}  & 97.1  & 89.3          & 81.9         & 85.4 & (4)       & 89.7   & 82.8          & 75.7         & 79.1  & (4)       \\ 
& \shortprop & 96.4($\downarrow$\red{0.7}) & 86.8 & 79.8 & 83.1($\downarrow$\red{2.3}) & (4) & 86.7($\downarrow$\red{3.0}) & 75.7 & 69.9 & 72.7($\downarrow$\red{6.4}) & (3)  \\ \cmidrule{2-12}

\multirow{2}{*}{\cite{blloshmi2021generating}$_{\text{flat}}$} & \multicolumn{1}{l}{CoNLL09}  & 97.4  &  90.9         &  89.6        & \textbf{90.2}  &   (1)    & 90.1   & 83.9          & 82.1         & 83.0 & (2)        \\ 
& \shortprop &  96.9($\downarrow$\red{0.5}) &     88.6     &     87.4    &   \underline{\textbf{88.0}}($\downarrow$\red{2.2}) &   (1)   & 87.8($\downarrow$\red{2.3})   & 77.6        & 76.3         & \underline{\textbf{76.9}}($\downarrow$\red{6.1}) & (1)  \\ \cmidrule{2-12}

% \multicolumn{10}{l}{\small{\underline{\textit{In-house: RoBERTa-base}}}} \\  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token\\ Classification\end{tabular}} 
\multirow{2}{*}{\cite{jindal-EtAl:2022:LREC}} & \multicolumn{1}{l}{CoNLL09}  & 96.8  & 89.9          & 89.3         & 89.6 & (2)        & 89.8   & 82.9          & 83.1         & \textbf{83.02} & (1)        \\
& \shortprop &
                              95.5($\downarrow$\red{1.3})  & 86.8          & 86.3         & 86.55($\downarrow$\red{3.0})    & (3)      & 83.4($\downarrow$\red{6.4})   & 73.9          & 74.3         & 74.1($\downarrow$\red{8.9}) &(2)   \\
                              \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison of SoTA SRL models with \shortprop\ and CoNLL09 evaluation metrics on CoNLL09 dataset. (r) denotes the ranking of SRL models corresponding to the evaluation metric. \textbf{BOLD} shows the best model with CoNLL09 evaluation script and \underline{\textbf{BOLD}} shows the best SRL model with \shortprop.}
\label{tab:p_09}
\end{table*}



%%% Data set table
\begin{table}[tbhp]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccllll}
\toprule
\multicolumn{1}{c}{Dataset}                    & \multicolumn{1}{l}{Args} & \multicolumn{1}{l}{Train} & \multicolumn{1}{l}{Dev}  & \multicolumn{1}{l}{Test} & ood  \\ \midrule
\multicolumn{1}{c}{\multirow{2}{*}{CoNLL09}}   & \multicolumn{1}{l}{\pargcstar}   & \multicolumn{1}{l}{0.77}  & \multicolumn{1}{l}{1.05} & \multicolumn{1}{l}{0.88} & 1.15 \\ \cmidrule{2-6} 
\multicolumn{1}{c}{}                           & \multicolumn{1}{l}{\pargrstar}   & \multicolumn{1}{l}{1.98}  & \multicolumn{1}{l}{2.03} & \multicolumn{1}{l}{2.07} & 2.24 \\ \midrule
% \multicolumn{1}{|c|}{\multirow{2}{*}{CoNLL12}} & \multicolumn{1}{l|}{C-}   & \multicolumn{1}{l|}{0.90}  & \multicolumn{1}{l|}{1.02} & \multicolumn{1}{l|}{0.97} & x \\ \cline{2-6} 
% \multicolumn{1}{|c|}{}                           & \multicolumn{1}{l|}{R-}   & \multicolumn{1}{l|}{2.43}  & \multicolumn{1}{l|}{2.31} & \multicolumn{1}{l|}{2.34} & x \\ \hline
% \multicolumn{6}{|c|}{}                                                                                                                                                   \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{CoNLL05}}   & \multicolumn{1}{l}{\pargcstar}   & \multicolumn{1}{l}{1.22}  & \multicolumn{1}{l}{1.24} & \multicolumn{1}{l}{1.71} & 0.91 \\ \cmidrule{2-6} 
\multicolumn{1}{c}{}                           & \multicolumn{1}{l}{\pargrstar}   & \multicolumn{1}{l}{3.26}  & \multicolumn{1}{l}{3.36} & \multicolumn{1}{l}{3.38} & 2.91 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Representation of \pargcstar\ and \pargrstar\ arguments in each split of different SRL datasets.}
\label{tab:dataset}
\end{table}

==> Performance measure metric for SRL/compare_table_05.tex <==
\begin{table*}[tbhp]
\centering
\begin{adjustbox}{width=0.9\linewidth}
\begin{tabular}{ccllllllllll}
\toprule
\multirow{3}{*}{Model}        & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Evaluation\\ script\end{tabular}}   & \multicolumn{5}{c}{In-domain}                       & \multicolumn{5}{c}{Out-of-domain}                    \\ \cmidrule(lr){3-7} \cmidrule(lr){8-12}
                              &                              & \multicolumn{1}{c}{PSD}   & \multicolumn{3}{c}{Argument Classification} &    & \multicolumn{1}{c}{PSD}    & \multicolumn{3}{c}{Argument Classification}     & \\  \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){8-8} \cmidrule(lr){9-11}
                              &                              & \multicolumn{1}{c}{F1}    & P             & R            & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{(r)}       & \multicolumn{1}{c}{F1}     & P             & R            & \multicolumn{1}{c}{F1}   & \multicolumn{1}{c}{(r)}        \\ \midrule
\multirow{2}{*}{\cite{zhang2021semantic}$_{\text{crf}}$} & \multicolumn{1}{l}{CoNLL05}  & 100   & 86.5          & 88.3           & 87.4 & (3)         & 100    & 79.0          & 81.1         & 80.0    & (3)     \\
                              & \multicolumn{1}{l}{\shortprop} & 100   & 86.1          & 87.8        & 87.03($\downarrow$\red{0.4}) & (2)           & 100    & 78.7          & 80.8         & 79.7($\downarrow$\red{0.3}) & (2)     \\  \cmidrule{2-12}
\multirow{2}{*}{\cite{zhang2021semantic}$_{\text{crf2o}}$} & \multicolumn{1}{l}{CoNLL05}  & 100   & 86.9          & 88.6           & 87.7 & (2)         & 100    & 78.9          & 81.2         &80.03    & (2)     \\
                              & \multicolumn{1}{l}{\shortprop} & 100   & 86.5          & 88.1         & \underline{\textbf{87.3}}($\downarrow$\red{0.4})& (1)           & 100    & 78.5          & 80.8         & 79.6($\downarrow$\red{0.4}) & (3)   \\   \cmidrule{2-12}
\multirow{2}{*}{\cite{jindal-EtAl:2022:LREC}} & \multicolumn{1}{l}{CoNLL05}  & 100   & 87.4          & 88.0           & \textbf{87.74} & (1)        & 100    & 80.4          & 81.4         & \textbf{80.9}  & (1)       \\
                              & \multicolumn{1}{l}{\shortprop} & 100   & 86.8          & 87.1         & 87.0($\downarrow$\red{0.7}) & (3)          & 100    & 79.7          & 80.5         & \underline{\textbf{80.1}}($\downarrow$\red{0.8})& (1)    \\  
                              \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison of SoTA SRL models with \shortprop\ and CoNLL05 evaluation metrics on CoNLL05 dataset. (r) denotes the ranking of SRL models corresponding to the evaluation metric. \textbf{BOLD} shows the best model with CoNLL05 evaluation script and \underline{\textbf{BOLD}} shows the best SRL model with \shortprop.}
\label{tab:p_05}
\end{table*}

==> Performance measure metric for SRL/cstar_table.tex <==

%%% Table 2
\begin{table}[]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{llllllllllll}
\multicolumn{12}{l}{\# text = Many confusing questions have been taxing my mind for years about Egypt and its people .}
\\ \hline
\multicolumn{1}{|l|}{ID}                & \multicolumn{1}{l|}{FORM}                                                                        & \multicolumn{1}{l|}{F}                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}PRED\\ SENSE\end{tabular}} & \multicolumn{1}{l|}{Gold} & \multicolumn{1}{l|}{P1}   & \multicolumn{1}{l|}{P2}   & \multicolumn{1}{l|}{P3}   & \multicolumn{1}{l|}{P4}   & \multicolumn{1}{l|}{P5}   & \multicolumn{1}{l|}{P6}   & \multicolumn{1}{l|}{P7}   \\ \hline
\multicolumn{1}{|l|}{1}                 & \multicolumn{1}{l|}{Many}                                                                        & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{2}                 & \multicolumn{1}{l|}{confusing}                                                                   & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{3}                 & \multicolumn{1}{l|}{questions}                                                                   & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\parg{0}}   & \multicolumn{1}{l|}{\parg{0}}   & \multicolumn{1}{l|}{\red{\textit{\parg{1}}}}   & \multicolumn{1}{l|}{\red{\textit{\parg{1}}}}   & \multicolumn{1}{l|}{\red{\textit{\pargc{0}}}} & \multicolumn{1}{l|}{\red{\textit{\parg{1}}}}   & \multicolumn{1}{l|}{\red{\textit{\pargc{0}}}} & \multicolumn{1}{l|}{\red{\textit{\pargc{0}}}} \\ \hline
\multicolumn{1}{|l|}{4}                 & \multicolumn{1}{l|}{have}                                                                        & \multicolumn{1}{l|}{Y}                  & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{5}                 & \multicolumn{1}{l|}{been}                                                                        & \multicolumn{1}{l|}{Y}                  & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{}     \\ \hline
\multicolumn{1}{|l|}{6}                 & \multicolumn{1}{l|}{taxing}                                                                      & \multicolumn{1}{l|}{Y}                  & \multicolumn{1}{l|}{tax.01}                                               & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{7}                 & \multicolumn{1}{l|}{my}                                                                          & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{8}                 & \multicolumn{1}{l|}{mind}                                                                        & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   & \multicolumn{1}{l|}{\parg{2}}   \\ \hline
\multicolumn{1}{|l|}{9}                 & \multicolumn{1}{l|}{for}                                                                         & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{10}                & \multicolumn{1}{l|}{years}                                                                       & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  & \multicolumn{1}{l|}{\texttt{TMP}}  \\ \hline
\multicolumn{1}{|l|}{11}                & \multicolumn{1}{l|}{about}                                                                       & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{12}                & \multicolumn{1}{l|}{Egypt}                                                                       & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\pargc{0}} & \multicolumn{1}{l|}{\red{\textit{\pargc{1}}}} & \multicolumn{1}{l|}{\pargc{0}} & \multicolumn{1}{l|}{\red{\textit{\pargc{1}}}} & \multicolumn{1}{l|}{\red{\textit{\parg{0}}}}   & \multicolumn{1}{l|}{\red{\textit{\pargc{2}}}} & \multicolumn{1}{l|}{\pargc{0}} & \multicolumn{1}{l|}{\red{\_}}   \\ \hline
\multicolumn{1}{|l|}{13}                & \multicolumn{1}{l|}{and}                                                                         & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{14}                & \multicolumn{1}{l|}{its}                                                                         & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{15}                & \multicolumn{1}{l|}{people}                                                                      & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{16}                & \multicolumn{1}{l|}{.}                                                                           & \multicolumn{1}{l|}{\_}                 & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{12}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \cline{2-12} 
\multicolumn{1}{c|}{\multirow{11}{*}{}} & \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ HEAD \\ Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{R}} & \multicolumn{1}{l|}{Conll09}                                              & \multicolumn{1}{l|}{4/4}  & \multicolumn{1}{l|}{3/4}  & \multicolumn{1}{l|}{3/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{3/4}  & \multicolumn{1}{l|}{2/4}  \\ \cline{4-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c|}{}                   & \multicolumn{1}{l|}{\shortprop}                                              & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{\cellgreen{2/3}}  & \multicolumn{1}{l|}{\cellgreen{2/3}}  & \multicolumn{1}{l|}{\cellgreen{2/3}}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{\cellgreen{2/3}}  \\ \cline{3-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{10}{c|}{}                                                                                                                                                                                                                                                                                                                              \\ \cline{3-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c|}{\multirow{2}{*}{P}} & \multicolumn{1}{l|}{Conll09}                                              & \multicolumn{1}{l|}{4/4}  & \multicolumn{1}{l|}{3/4}  & \multicolumn{1}{l|}{3/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{3/4}  & \multicolumn{1}{l|}{2/3}  \\ \cline{4-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c|}{}                   & \multicolumn{1}{l|}{\shortprop}                                              & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{\cellgreen{2/4}}  & \multicolumn{1}{l|}{\cellgreen{2/4}}  & \multicolumn{1}{l|}{\cellgreen{2/3}}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{\cellgreen{2/3}}  \\ \cline{2-12} 
\multicolumn{1}{c}{}                   & \multicolumn{11}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \cline{2-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ SPAN\\  Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{R}} & \multicolumn{1}{l|}{Conll05}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  \\\cline{4-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c|}{}                   & \multicolumn{1}{l|}{\shortprop}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{2/3}  \\ \cline{3-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{10}{c|}{}                                                                                                                                                                                                                                                                                                                              \\ \cline{3-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c|}{\multirow{2}{*}{P}} & \multicolumn{1}{l|}{Conll05}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  \\  \cline{4-12} 
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c|}{}                   & \multicolumn{1}{l|}{\shortprop}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/4}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{\cellgreen{3/3}}  & \multicolumn{1}{l|}{2/3}  \\ \cline{2-12} 
\end{tabular}

\end{adjustbox}
\caption{Comparing evaluation metrics on 7 examples, showing the effect of \pargcstar\ labels. %\red{\textit{RED}} shows a wrong prediction by  a hypothetical model. {\green{GREEN}} cell highlights where \shortprop\ differs from existing metrics.}
\red{\textit{RED-italic}} and {\green{GREEN}} cell are used in the same manner as Table~\ref{tab:pred_sense}.}
\label{tab:example_c}
\end{table}

==> Performance measure metric for SRL/existing-eval.tex <==
%\section{Existing evaluation metrics for SRL}\label{sec:metrics}

Most of the existing evaluation metrics came from shared tasks for the development of systems capable of extracting predicates and arguments from natural language sentences. In this section, we summarize the approaches to SRL evaluation in the shared tasks from SemEval and CoNLL

\subsection{Senseval and SemEval}


SemEval (Semantic Evaluation) is a series of evaluations of computational semantic analysis systems that evolved from the Senseval (word sense evaluation) series. 

\textbf{SENSEVAL-3} \cite{litkowski-2004-senseval} addressed the task of automatic labeling of semantic roles and was designed to encourage research into and use of the FrameNet dataset. 
The system would receive as input a target word and its frame, and was required to identify and label the frame elements (arguments). The evaluation metric counted the number of arguments correctly identified (complete match of span) and labeled, but did not penalize those spuriously identified.  An overlap score was generated as the average of proportion of partial matches.

\textbf{SemEval-2007} contained three tasks that evaluate SRL. 
Task 17 and 18 identified arguments for given predicates using two different role label sets: PropBank and VerbNet \cite{pradhan-etal-2007-semeval}. 
They used the \verb|srl-eval.pl| script from the CoNLL-2005 scoring package \cite{carreras-marquez-2005-introduction} (see below).  
Task 19 consists of recognizing words and phrases that evoke semantic frames from FrameNet and their semantic dependents, which are usually, but not always, their syntactic dependents. The evaluation measured precision and recall for frames and frame elements, with partial credit for incorrect but closely related frames. Two types of evaluation were carried out. The first is the label matching evaluation. The participant's labeled data were compared directly with the gold standard labeled using the same evaluation procedure used in the previous SRL tasks at SemEval. The second is the semantic dependency evaluation, in which both the gold standard and the submitted data were first converted to semantic dependency graphs and compared. 
% Task 19 recognized semantic frames from FrameNet and their semantic dependents.
% It used the same evaluation method as above based on span comparison, and also compared the outputs converted into semantic dependency graphs. 


\textbf{SemEval-2012} \cite{kordjamshidi-etal-2012-semeval} and \textbf{SemEval-2013} \cite{kolomiyets-etal-2013-semeval} introduced the `Spatial Role Labeling' task, but this is somewhat different from the standard SRL task and will not be discussed in this paper. Since \textbf{SemEval-2014} \cite{marelli-etal-2014-semeval}, a deeper semantic representation of sentences in a single graph-based structure via semantic parsing has superseded  the previous `shallow' SRL tasks.

\subsection{CoNLL}

The \textbf{CoNLL-2004} shared task \cite{carreras-marquez-2004-introduction} was based on the PropBank corpus, comprising six sections of the Wall Street Journal part of the Penn Treebank \cite{kingsbury-palmer-2002-treebank} enriched with predicate–argument structures. 
The task was to identify and label the arguments of each marked verb. The precision, recall and F1 of arguments were evaluated using the \verb|srl-eval.pl| program. For an argument to be correctly recognized, the words spanning the argument as well as its semantic role have to be correct. The verb argument is the lexicalization of the predicate of the proposition. Most of the time, the verb corresponds to the target verb of the proposition, which is provided as input, and only in few cases the verb participant spans more words than the target verb. This situation makes the verb easy to identify and, since there is one verb with each proposition, evaluating its recognition overestimates the overall performance of a system. For this reason, the verb argument is excluded from evaluation. The shared task proceedings does not details how non-continuous arguments are evaluated. In \textbf{CoNLL-2005} \cite{carreras2005introduction} a system had to recognize and label the arguments of each target verb. The evaluation method remained the same as CoNLL-2004, using the same evaluation code. 

The \textbf{CoNLL 2008} shared task \cite{surdeanu-etal-2008-conll} was dedicated to the joint parsing of syntactic and semantic dependencies. The shared task was divided into three subtasks: (i) parsing of syntactic dependencies, (ii) identification and disambiguation of semantic predicates, and (iii) identification of arguments and assignment of semantic roles for each predicate. SRL was performed and evaluated using a dependency-based representation for both syntactic and semantic dependencies. 

The official evaluation measures consist of three different scores: (i) syntactic dependencies are scored using the labeled attachment score (LAS),
(ii) semantic dependencies are evaluated using a labeled F1 score, and (iii) the overall task is scored with a macro average of the two previous scores. The semantic propositions are evaluated by converting them to semantic dependencies, i.e., a semantic dependency from every predicate
to all its individual arguments were created. These dependencies are labeled with the labels of the corresponding arguments. Additionally, a semantic dependency from each predicate to a virtual
ROOT node was created. The latter dependencies are labeled with the predicate senses. This approach guarantees that the semantic dependency structure conceptually forms a single-rooted, connected (not necessarily acyclic) graph. More importantly, this scoring strategy implies that if a system assigns the incorrect predicate sense, it still receives some points for the arguments correctly assigned. Several additional evaluation measures were applied to further analyze the performance of the participating systems. The \emph{Exact Match} reports the percentage of sentences that are completely correct, i.e., all the generated syntactic dependencies are correct and all the semantic propositions are present and correct. The \emph{Perfect Proposition F1} score entire semantic frames or propositions. The ratio between labeled F1 score for semantic dependencies and the LAS for syntactic dependencies.

As in CoNLL-2008, the CoNLL-2009 shared task \cite{hajic-etal-2009-conll} combined syntactic dependency parsing and the task of identifying and labeling semantic arguments of verbs or nouns for six more languages in addition to the original English from CoNLL-2008. Predicate disambiguation was still part of the task, whereas the identification of argument-bearing words was not. This decision was made to compensate for the significant differences between languages and between the annotation schemes used. The evaluation of SRL was done similar to CoNLL-2008.



==> Performance measure metric for SRL/psd_table.tex <==

%%%% Table 1
\begin{table}[]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{|ccclllll|}
\multicolumn{8}{l}{\#   text = Yesterday, John bought a car.} 
\\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{FORM}} & \multicolumn{1}{c|}{\multirow{2}{*}{FLAG}}                                                    & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}PRED\\ SENSE\end{tabular}}} & \multicolumn{4}{c|}{Predicate-argument prediction}                         \\ \cline{5-8} 
\multicolumn{1}{|c|}{}                    & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{c|}{}                                                                      & %\multicolumn{1}{l|}{buy.01} & \multicolumn{1}{l|}{\red{buy\_out.03}} & \multicolumn{1}{l|}{\red{buy.05}} & \red{sell.01} \\ \hline
\multicolumn{1}{l|}{Gold} & \multicolumn{1}{l|}{P1} & \multicolumn{1}{l|}{P2} & P3 \\ \hline
\multicolumn{1}{|l|}{1}                   & \multicolumn{1}{l|}{Yesterday}              & \multicolumn{1}{l|}{\_}                                                                       & \multicolumn{1}{l|}{\_}                                                                    & \multicolumn{1}{l|}{\texttt{TMP}} & \multicolumn{1}{l|}{\texttt{TMP}}      & \multicolumn{1}{l|}{\texttt{TMP}} & \texttt{TMP} \\ \hline
\multicolumn{1}{|l|}{2}                   & \multicolumn{1}{l|}{,}                      & \multicolumn{1}{l|}{\_}                                                                       & \multicolumn{1}{l|}{\_}                                                                    & \multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}    & \_  \\ \hline
\multicolumn{1}{|l|}{3}                   & \multicolumn{1}{l|}{John}                   & \multicolumn{1}{l|}{\_}                                                                       & \multicolumn{1}{l|}{\_}                                                                    & \multicolumn{1}{l|}{\parg{0}}     & \multicolumn{1}{l|}{\parg{0}}          & \multicolumn{1}{l|}{\parg{0}}  & \parg{0}     \\ \hline
\multicolumn{1}{|l|}{4}                   & \multicolumn{1}{l|}{bought}                 & \multicolumn{1}{l|}{Y}                                                                        & \multicolumn{1}{l|}{buy.01}                                                                & 
\multicolumn{1}{l|}{buy.01} & \multicolumn{1}{l|}{\red{\textit{buy\_out.03}}} & \multicolumn{1}{l|}{\red{\textit{buy.05}}} & \red{\textit{sell.01}} \\ \hline
%\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_   \\ \hline
\multicolumn{1}{|l|}{5}                   & \multicolumn{1}{l|}{a}                      & \multicolumn{1}{l|}{\_}                                                                       & \multicolumn{1}{l|}{\_}                                                                    & \multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_   \\ \hline
\multicolumn{1}{|l|}{6}                   & \multicolumn{1}{l|}{car}                    & \multicolumn{1}{l|}{\_}                                                                       & \multicolumn{1}{l|}{\_}                                                                    & \multicolumn{1}{l|}{\parg{1}}     & \multicolumn{1}{l|}{\parg{1}}          & \multicolumn{1}{l|}{\parg{1}}    & \parg{1}  \\ \hline
\multicolumn{1}{|l|}{7}                   & \multicolumn{1}{l|}{.}                      & \multicolumn{1}{l|}{\_}                                                                       & \multicolumn{1}{l|}{\_}                                                                    & \multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_  \\ \hline
\multicolumn{1}{c}{}                     & \multicolumn{7}{c}{}                                                                                                                                                                                                                                                                                              \\ 
\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Predicate \\ Evaluation\end{tabular}}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{R}}                                             
    & \multicolumn{1}{l|}{CoNLL05}                                                                     & \multicolumn{4}{c|}{do not evaluate}                                                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{CoNLL09}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}      & \multicolumn{1}{l|}{0/1}     & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{\shortprop}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}    & \multicolumn{1}{l|}{0/1}       & \cellgreen{0/1}      \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{P}}                                                 & \multicolumn{1}{l|}{CoNLL05}                                                                     & \multicolumn{4}{c|}{do not evaluate}                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{} &                                                                    \multicolumn{1}{l|}{CoNLL09}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}   & \multicolumn{1}{l|}{0/1}       & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                & \multicolumn{1}{l|}{\shortprop}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}    & \multicolumn{1}{l|}{0/1}       & \cellgreen{0/1}      \\ \cline{2-8} 
\multicolumn{8}{l}{}\\
%\multicolumn{6}{c|}{}                     
% & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                                                                         & \multicolumn{1}{l|}{}                                                                      & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}            &        
% \multicolumn{1}{c|}{\multirow{15}{*}{}}   & \multicolumn{6}{c|}{\multirow{2}{*}{}}      
\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{R}}                                                 & \multicolumn{1}{l|}{CoNLL05}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3} & 0/3                                                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{CoNLL09} &                                                                     \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{3/3}        & 3/3      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{\shortprop}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}}   & \multicolumn{1}{l|}{\cellgreen{1/3}}      & \cellgreen{1/3}      \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{P}}                                                 & \multicolumn{1}{l|}{CoNLL05}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3}       & 0/3                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{} &                                                                    \multicolumn{1}{l|}{CoNLL09}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3} & \multicolumn{1}{l|}{3/3}         & 3/3      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                & \multicolumn{1}{l|}{\shortprop}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}} & \multicolumn{1}{l|}{\cellgreen{1/3}}        &  \cellgreen{1/3}      \\ \cline{2-8} %
\end{tabular}
\end{adjustbox}
\caption{Comparing evaluation metrics on 4 examples, showing the effect of wrong predicate sense on argument label evaluation. \red{\textit{RED-italic}} shows a wrong prediction by  a hypothetical model. {\green{GREEN}} cell highlights where \shortprop\ differs from existing metrics.}
\label{tab:pred_sense}
\end{table}

\begin{comment}
\multicolumn{1}{c}{}                     & \multicolumn{7}{c}{}                                                                                                                                                                                                                                                                                              \\ 

\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{8}{*}{Sense}} & \multicolumn{1}{c|}{\multirow{2}{*}{CoNLL09}}                                                 & \multicolumn{1}{l|}{P}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}   & \multicolumn{1}{l|}{0}       & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{R}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}      & \multicolumn{1}{l|}{0}     & 1/1      \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{CoNLL05}}                                                 & \multicolumn{1}{l|}{P}                                                                     & \multicolumn{4}{c|}{\multirow{2}{*}{do not evaluate}}                   \\ \cline{4-4}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{R}                                                                     & \multicolumn{4}{c|}{}                                                   \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{Proposed}}                                                & \multicolumn{1}{l|}{P}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}    & \multicolumn{1}{l|}{0}       & \cellgreen{0}      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{R}                                                                     & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}    & \multicolumn{1}{l|}{0}       & \cellgreen{0}      \\ \cline{2-8}

\multicolumn{6}{c|}{}                     
% & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                                                                         & \multicolumn{1}{l|}{}                                                                      & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}            &        

\\ 

\cline{2-8} 

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{8}{*}{Args}}  & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CoNLL09\\ Head\end{tabular}}}  & \multicolumn{1}{l|}{P}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3} & \multicolumn{1}{l|}{3/3}         & 3/3    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{R}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{3/3}        & 3/3    \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CoNLL05\\ Span\end{tabular}}}  & \multicolumn{1}{l|}{P}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3}       & 0/3    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{R}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}       & \multicolumn{1}{l|}{3/3}   & 0/3    \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Proposed\\ Head/Span \end{tabular}}} & \multicolumn{1}{l|}{P}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}} & \multicolumn{1}{l|}{\cellgreen{1/3}}        &  \cellgreen{1/3}    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                                         & \multicolumn{1}{l|}{R}                                                                     & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}}   & \multicolumn{1}{l|}{\cellgreen{1/3}}      & \cellgreen{1/3}    \\ \cline{2-8} 
\end{comment}


==> Performance measure metric for SRL/psd_table_to_edit.tex <==
\begin{table}[htbp]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{|c| c| c| l| l| l| l| l|}
\hline
& \multicolumn{6}{|l|}{\#   text = Yesterday, John bought a car.} 
\\ \hline

& \multicolumn{1}{|c|}{\multirow{2}{*}{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{FORM}} & %\multicolumn{1}{c|}{\multirow{2}{*}{FLAG}}  & 
%\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}PRED\\ SENSE\end{tabular}}} & 
\multicolumn{4}{c|}{Predicate sense prediction}                         
\\ \cline{4-7} 

& \multicolumn{1}{|c|}{}                    & \multicolumn{1}{c|}{}                       & 
%\multicolumn{1}{c|}{}                       & %\multicolumn{1}{c|}{}                    & %\multicolumn{1}{l|}{buy.01} & \multicolumn{1}{l|}{\red{buy\_out.03}} & \multicolumn{1}{l|}{\red{buy.05}} & \red{sell.01} \\ \hline
\multicolumn{1}{l|}{Gold} & \multicolumn{1}{l|}{P1} & \multicolumn{1}{l|}{P2} & P3 \\ \hline
& \multicolumn{1}{|l|}{1}                   & \multicolumn{1}{l|}{Yesterday}              & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{AM-TMP} & \multicolumn{1}{l|}{AM-TMP}      & \multicolumn{1}{l|}{AM-TMP} & AM-TMP 
\\ \hline

& \multicolumn{1}{|l|}{2}                   & \multicolumn{1}{l|}{,}                      & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}    & \_  
\\ \hline

& \multicolumn{1}{|l|}{3}                   & \multicolumn{1}{l|}{John}                   & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{A0}     & \multicolumn{1}{l|}{A0}          & \multicolumn{1}{l|}{A0}  & A0     
\\ \hline

& \multicolumn{1}{|l|}{4}                   & \multicolumn{1}{l|}{bought}                 & 
%\multicolumn{1}{l|}{Y}                      & \multicolumn{1}{l|}{buy.01}              & 
\multicolumn{1}{l|}{buy.01} & \multicolumn{1}{l|}{\red{buy\_out.03}} & \multicolumn{1}{l|}{\red{buy.05}} & \red{sell.01} 
\\ \hline

%\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_   \\ \hline
& \multicolumn{1}{|l|}{5}                   & \multicolumn{1}{l|}{a}                      & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_   
\\ \hline

& \multicolumn{1}{|l|}{6}                   & \multicolumn{1}{l|}{car}                    & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{A1}     & \multicolumn{1}{l|}{A1}          & \multicolumn{1}{l|}{A1}    & A1  
\\ \hline

& \multicolumn{1}{|l|}{7}                   & \multicolumn{1}{l|}{.}                      & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_  
\\ \hline

\multicolumn{1}{c}{}                     & \multicolumn{7}{c}{}                                                                                                                                                                                                                                                                                     
\\ \cline{1-7}

%\multicolumn{1}{c|}{}                     & 
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Predicate \\ Evaluation\end{tabular}}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{R}}                                             
    & \multicolumn{1}{l|}{CoNLL05}                   & \multicolumn{4}{c|}{do not evaluate}                                                   
\\ \cline{4-8}

%\multicolumn{1}{c|}{}                     & 
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{CoNLL09}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}      & \multicolumn{1}{l|}{0/1}     & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{Proposed}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}    & \multicolumn{1}{l|}{0/1}       & \cellgreen{0/1}      \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{P}}                                                 & \multicolumn{1}{l|}{CoNLL05}                   & \multicolumn{4}{c|}{do not evaluate}                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{} &                                                                    \multicolumn{1}{l|}{CoNLL09}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}   & \multicolumn{1}{l|}{0/1}       & 1/1      
\\ \cline{4-8} 

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                & \multicolumn{1}{l|}{Proposed}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}    & \multicolumn{1}{l|}{0/1}       & \cellgreen{0/1}      
\\ \cline{2-8} 

\multicolumn{8}{l}{}\\
%\multicolumn{6}{c|}{}                     
% & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}            &        
% \multicolumn{1}{c|}{\multirow{15}{*}{}}   & \multicolumn{6}{c|}{\multirow{2}{*}{}}      
\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{R}}                                                 & \multicolumn{1}{l|}{CoNLL05 Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3} & 0/3                                                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{CoNLL09 Head} &                                                                     \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{3/3}        & 3/3      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{Proposed Head/Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}}   & \multicolumn{1}{l|}{\cellgreen{1/3}}      & \cellgreen{1/3}      \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} 
\\ \cline{3-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{P}}                                                 & \multicolumn{1}{l|}{CoNLL05 Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3}       & 0/3                   
\\ \cline{4-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{} &                                                                    \multicolumn{1}{l|}{CoNLL09 Head}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3} & \multicolumn{1}{l|}{3/3}         & 3/3      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                & \multicolumn{1}{l|}{Proposed Head/Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}} & \multicolumn{1}{l|}{\cellgreen{1/3}}        &  \cellgreen{1/3}      
\\ \cline{2-8} %

\end{tabular}
\end{adjustbox}
\caption{Comparison of 3 evaluation metrics on 4 examples, showing effect of wrong predicate sense on argument label evaluation. \red{RED} denotes wrong prediction by  a hypothetical model. {\green{GREEN}} cell denotes the proposed eval is different from existing eval.}
\label{tab:pred_sense}
\end{table}

\begin{comment}
\multicolumn{1}{c}{}                     & \multicolumn{7}{c}{}                                                                                                                                                                                                                                                                                              \\ 

\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{8}{*}{Sense}} & \multicolumn{1}{c|}{\multirow{2}{*}{CoNLL09}}                                                 & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}   & \multicolumn{1}{l|}{0}       & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}      & \multicolumn{1}{l|}{0}     & 1/1      \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{CoNLL05}}                                                 & \multicolumn{1}{l|}{P}                   & \multicolumn{4}{c|}{\multirow{2}{*}{do not evaluate}}                   \\ \cline{4-4}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{4}{c|}{}                                                   \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{Proposed}}                                                & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}    & \multicolumn{1}{l|}{0}       & \cellgreen{0}      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}    & \multicolumn{1}{l|}{0}       & \cellgreen{0}      \\ \cline{2-8}

\multicolumn{6}{c|}{}                     
% & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}            &        

\\ 

\cline{2-8} 

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{8}{*}{Args}}  & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CoNLL09\\ Head\end{tabular}}}  & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3} & \multicolumn{1}{l|}{3/3}         & 3/3    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{3/3}        & 3/3    \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CoNLL05\\ Span\end{tabular}}}  & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3}       & 0/3    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}       & \multicolumn{1}{l|}{3/3}   & 0/3    \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Proposed\\ Head/Span \end{tabular}}} & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}} & \multicolumn{1}{l|}{\cellgreen{1/3}}        &  \cellgreen{1/3}    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}}   & \multicolumn{1}{l|}{\cellgreen{1/3}}      & \cellgreen{1/3}    \\ \cline{2-8} 
\end{comment}


==> Performance measure metric for SRL/rstar_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%%% Table 3
\begin{table}[]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{lllllllllll}
\multicolumn{11}{l}{\# text = This is exactly a road that leads nowhere.}
\\ \hline
\multicolumn{1}{|l|}{ID}               & \multicolumn{1}{l|}{FORM}                                                                        & \multicolumn{1}{l|}{F}                       & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}PRED\\ SENSE\end{tabular}} & \multicolumn{1}{l|}{Gold} & \multicolumn{1}{l|}{P1}   & \multicolumn{1}{l|}{P2}   & \multicolumn{1}{l|}{P3}   & \multicolumn{1}{l|}{P4}   & \multicolumn{1}{l|}{P5}   & \multicolumn{1}{l|}{P6}   \\ \hline
\multicolumn{1}{|l|}{1}                & \multicolumn{1}{l|}{This}                                                                        & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{2}                & \multicolumn{1}{l|}{is}                                                                          & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{3}                & \multicolumn{1}{l|}{exactly}                                                                     & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{4}                & \multicolumn{1}{l|}{a}                                                                           & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\red{\textit{\parg{0}}}}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{5}                & \multicolumn{1}{l|}{road}                                                                        & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\parg{0}}   & \multicolumn{1}{l|}{\red{\textit{\parg{1}}}}   & \multicolumn{1}{l|}{\parg{0}}   & \multicolumn{1}{l|}{\red{\textit{\parg{1}}}}   & \multicolumn{1}{l|}{\red{\textit{\_}}}   & \multicolumn{1}{l|}{\red{\textit{\pargr{0}}}} & \multicolumn{1}{l|}{\red{\textit{\pargr{0}}}} \\ \hline
\multicolumn{1}{|l|}{6}                & \multicolumn{1}{l|}{that}                                                                        & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\pargr{0}} & \multicolumn{1}{l|}{\pargr{0}} & \multicolumn{1}{l|}{\red{\textit{\pargr{1}}}} & \multicolumn{1}{l|}{\red{\textit{\pargr{1}}}} & \multicolumn{1}{l|}{\pargr{0}} & \multicolumn{1}{l|}{\pargr{0}} & \multicolumn{1}{l|}{\red{\textit{\parg{0}}}}   \\ \hline
\multicolumn{1}{|l|}{7}                & \multicolumn{1}{l|}{leads}                                                                       & \multicolumn{1}{l|}{Y}                          & \multicolumn{1}{l|}{lead.01}                                              & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{|l|}{8}                & \multicolumn{1}{l|}{nowhere}                                                                     & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\parg{4}}   & \multicolumn{1}{l|}{\parg{4}}   & \multicolumn{1}{l|}{\parg{4}}   & \multicolumn{1}{l|}{\parg{4}}   & \multicolumn{1}{l|}{\parg{4}}   & \multicolumn{1}{l|}{\parg{4}}   & \multicolumn{1}{l|}{\parg{4}}   \\ \hline
\multicolumn{1}{|l|}{9}                & \multicolumn{1}{l|}{.}                                                                           & \multicolumn{1}{l|}{\_}                         & \multicolumn{1}{l|}{\_}                                                   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   & \multicolumn{1}{l|}{\_}   \\ \hline
\multicolumn{1}{c}{\multirow{10}{*}{}} & \multicolumn{10}{c}{} \\ 
\cline{2-11} 
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ HEAD \\ Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{R}}    & \multicolumn{1}{l|}{Conll09}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  \\ \cline{4-11} 
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{}                                                                            & \multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{\shortprop}                                             & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{1/3}  \\ \cline{3-11} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{9}{c|}{} \\ \cline{3-11}

\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{}                                                                            & \multicolumn{1}{c|}{\multirow{2}{*}{P}} & \multicolumn{1}{l|}{Conll09}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  \\ \cline{4-11} 
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{}                                                                            & \multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{\shortprop}                                             & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{1/3}  \\ \cline{2-11} 
\multicolumn{1}{c}{}                   & \multicolumn{10}{c}{}\\ 
\cline{2-11} 
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ SPAN\\  Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{R}}    & \multicolumn{1}{l|}{Conll05}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{1/3}  \\ \cline{4-11} 
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{}                                                                            & \multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{\shortprop}                                             & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{1/3}  \\ \cline{3-11} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{9}{c|}{} \\ \cline{3-11}
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{}                                                                            & \multicolumn{1}{c|}{\multirow{2}{*}{P}} & \multicolumn{1}{l|}{Conll05}                                              & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{1/3}  \\ \cline{4-11} 
\multicolumn{1}{c}{}                   & \multicolumn{1}{|c|}{}                                                                            & \multicolumn{1}{c|}{}                           & \multicolumn{1}{l|}{\shortprop}                                             & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{2/3}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{\cellgreen{1/3}}  & \multicolumn{1}{l|}{1/3}  & \multicolumn{1}{l|}{1/3}  \\ \cline{2-11} 
\end{tabular}
\end{adjustbox}
\caption{Comparing evaluation metrics on 6 examples, showing the effect of \pargrstar\ labels. %Illustrating the issues with different evaluation scripts. Here it is assumed that the arguments are predicted correctly, even the predicate sense is wrong. 
%\red{RED} shows a wrong prediction by a hypothetical model. {\green{GREEN}} cell highlights where \shortprop\ differs from existing metrics.}
\red{\textit{RED-italic}} and {\green{GREEN}} cell are used in the same manner as Table~\ref{tab:pred_sense}.}
\label{tab:example_r}
\end{table}

==> psd_table_to_edit.tex <==
\begin{table}[htbp]
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{|c| c| c| l| l| l| l| l|}
\hline
& \multicolumn{6}{|l|}{\#   text = Yesterday, John bought a car.} 
\\ \hline

& \multicolumn{1}{|c|}{\multirow{2}{*}{ID}} & \multicolumn{1}{c|}{\multirow{2}{*}{FORM}} & %\multicolumn{1}{c|}{\multirow{2}{*}{FLAG}}  & 
%\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}PRED\\ SENSE\end{tabular}}} & 
\multicolumn{4}{c|}{Predicate sense prediction}                         
\\ \cline{4-7} 

& \multicolumn{1}{|c|}{}                    & \multicolumn{1}{c|}{}                       & 
%\multicolumn{1}{c|}{}                       & %\multicolumn{1}{c|}{}                    & %\multicolumn{1}{l|}{buy.01} & \multicolumn{1}{l|}{\red{buy\_out.03}} & \multicolumn{1}{l|}{\red{buy.05}} & \red{sell.01} \\ \hline
\multicolumn{1}{l|}{Gold} & \multicolumn{1}{l|}{P1} & \multicolumn{1}{l|}{P2} & P3 \\ \hline
& \multicolumn{1}{|l|}{1}                   & \multicolumn{1}{l|}{Yesterday}              & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{AM-TMP} & \multicolumn{1}{l|}{AM-TMP}      & \multicolumn{1}{l|}{AM-TMP} & AM-TMP 
\\ \hline

& \multicolumn{1}{|l|}{2}                   & \multicolumn{1}{l|}{,}                      & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}    & \_  
\\ \hline

& \multicolumn{1}{|l|}{3}                   & \multicolumn{1}{l|}{John}                   & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{A0}     & \multicolumn{1}{l|}{A0}          & \multicolumn{1}{l|}{A0}  & A0     
\\ \hline

& \multicolumn{1}{|l|}{4}                   & \multicolumn{1}{l|}{bought}                 & 
%\multicolumn{1}{l|}{Y}                      & \multicolumn{1}{l|}{buy.01}              & 
\multicolumn{1}{l|}{buy.01} & \multicolumn{1}{l|}{\red{buy\_out.03}} & \multicolumn{1}{l|}{\red{buy.05}} & \red{sell.01} 
\\ \hline

%\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_   \\ \hline
& \multicolumn{1}{|l|}{5}                   & \multicolumn{1}{l|}{a}                      & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_   
\\ \hline

& \multicolumn{1}{|l|}{6}                   & \multicolumn{1}{l|}{car}                    & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{A1}     & \multicolumn{1}{l|}{A1}          & \multicolumn{1}{l|}{A1}    & A1  
\\ \hline

& \multicolumn{1}{|l|}{7}                   & \multicolumn{1}{l|}{.}                      & 
%\multicolumn{1}{l|}{\_}                     & \multicolumn{1}{l|}{\_}                  & 
\multicolumn{1}{l|}{\_}     & \multicolumn{1}{l|}{\_}          & \multicolumn{1}{l|}{\_}   & \_  
\\ \hline

\multicolumn{1}{c}{}                     & \multicolumn{7}{c}{}                                                                                                                                                                                                                                                                                     
\\ \cline{1-7}

%\multicolumn{1}{c|}{}                     & 
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Predicate \\ Evaluation\end{tabular}}} & 
\multicolumn{1}{c|}{\multirow{3}{*}{R}}                                             
    & \multicolumn{1}{l|}{CoNLL05}                   & \multicolumn{4}{c|}{do not evaluate}                                                   
\\ \cline{4-8}

%\multicolumn{1}{c|}{}                     & 
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{CoNLL09}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}      & \multicolumn{1}{l|}{0/1}     & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{Proposed}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}    & \multicolumn{1}{l|}{0/1}       & \cellgreen{0/1}      \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{P}}                                                 & \multicolumn{1}{l|}{CoNLL05}                   & \multicolumn{4}{c|}{do not evaluate}                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{} &                                                                    \multicolumn{1}{l|}{CoNLL09}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}   & \multicolumn{1}{l|}{0/1}       & 1/1      
\\ \cline{4-8} 

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                & \multicolumn{1}{l|}{Proposed}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0/1}    & \multicolumn{1}{l|}{0/1}       & \cellgreen{0/1}      
\\ \cline{2-8} 

\multicolumn{8}{l}{}\\
%\multicolumn{6}{c|}{}                     
% & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}            &        
% \multicolumn{1}{c|}{\multirow{15}{*}{}}   & \multicolumn{6}{c|}{\multirow{2}{*}{}}      
\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Argument \\ Evaluation\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{R}}                                                 & \multicolumn{1}{l|}{CoNLL05 Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3} & 0/3                                                   \\ \cline{4-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{CoNLL09 Head} &                                                                     \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{3/3}        & 3/3      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{Proposed Head/Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}}   & \multicolumn{1}{l|}{\cellgreen{1/3}}      & \cellgreen{1/3}      \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} 
\\ \cline{3-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{3}{*}{P}}                                                 & \multicolumn{1}{l|}{CoNLL05 Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3}       & 0/3                   
\\ \cline{4-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{} &                                                                    \multicolumn{1}{l|}{CoNLL09 Head}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3} & \multicolumn{1}{l|}{3/3}         & 3/3      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                                & \multicolumn{1}{l|}{Proposed Head/Span}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}} & \multicolumn{1}{l|}{\cellgreen{1/3}}        &  \cellgreen{1/3}      
\\ \cline{2-8} %

\end{tabular}
\end{adjustbox}
\caption{Comparison of 3 evaluation metrics on 4 examples, showing effect of wrong predicate sense on argument label evaluation. \red{RED} denotes wrong prediction by  a hypothetical model. {\green{GREEN}} cell denotes the proposed eval is different from existing eval.}
\label{tab:pred_sense}
\end{table}

\begin{comment}
\multicolumn{1}{c}{}                     & \multicolumn{7}{c}{}                                                                                                                                                                                                                                                                                              \\ 

\cline{2-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{8}{*}{Sense}} & \multicolumn{1}{c|}{\multirow{2}{*}{CoNLL09}}                                                 & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}   & \multicolumn{1}{l|}{0}       & 1/1      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}      & \multicolumn{1}{l|}{0}     & 1/1      \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{CoNLL05}}                                                 & \multicolumn{1}{l|}{P}                   & \multicolumn{4}{c|}{\multirow{2}{*}{do not evaluate}}                   \\ \cline{4-4}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{4}{c|}{}                                                   \\ \cline{3-8}
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{Proposed}}                                                & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}    & \multicolumn{1}{l|}{0}       & \cellgreen{0}      \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{1/1}    & \multicolumn{1}{l|}{0}    & \multicolumn{1}{l|}{0}       & \cellgreen{0}      \\ \cline{2-8}

\multicolumn{6}{c|}{}                     
% & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}            &        

\\ 

\cline{2-8} 

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{\multirow{8}{*}{Args}}  & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CoNLL09\\ Head\end{tabular}}}  & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3} & \multicolumn{1}{l|}{3/3}         & 3/3    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}  & \multicolumn{1}{l|}{3/3}        & 3/3    \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}

\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CoNLL05\\ Span\end{tabular}}}  & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}   & \multicolumn{1}{l|}{3/3}       & 0/3    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{3/3}       & \multicolumn{1}{l|}{3/3}   & 0/3    \\ \cline{3-8} 
\multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        & \multicolumn{6}{c|}{} \\ \cline{3-8}
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Proposed\\ Head/Span \end{tabular}}} & \multicolumn{1}{l|}{P}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}} & \multicolumn{1}{l|}{\cellgreen{1/3}}        &  \cellgreen{1/3}    \\ \cline{4-8} 
\multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{l|}{R}                   & \multicolumn{1}{l|}{3/3}    & \multicolumn{1}{l|}{\cellgreen{1/3}}   & \multicolumn{1}{l|}{\cellgreen{1/3}}      & \cellgreen{1/3}    \\ \cline{2-8} 
\end{comment}

